SCOPE:Planning for Hybrid Querying over Clinical Trial Data

We study clinical trial table reasoning, where answers are not directly stored in visible cells but must be reasoned from semantic understanding through normalization, classification, extraction, or lightweight domain reasoning. Motivated by the observation that current LLM approaches often suffer from "bad reasoning" under implicit planning assumptions, we focus on settings in which the model must recover implicit attributes such as therapy type, added agents, endpoint roles, or follow-up status from partially observed clinical-trial tables. We propose SCOPE (Structured Clinical hybrid Planning for Evidence retrieval in clinical trials), a multi-LLM planner-based framework that decomposes the task into row selection, structured planning, and execution. The planner makes the source field, reasoning rules, and output constraints explicit before answer generation, reducing ambiguity relative to direct prompting. We evaluate SCOPE on 1,500 hybrid reasoning questions over oncology clinical-trial tables against zero-shot, few-shot, chain-of-thought, TableGPT2, Blend-SQL, and EHRAgent. Results show that explicit multi-LLM planning improves accuracy for reasoning-based questions while offering a stronger accuracy-efficiency tradeoff than heavier agentic baselines. Our findings position clinical trial reasoning as a distinct table understanding problem and highlight hybrid planner-based decomposition as an effective solution

==> prompts/cot.tex <==
You are an expert table reasoning agent.
The task is to answer cancer drug trial questions using only the visible CSV table.

You MUST follow the reasoning scaffold below, but do NOT show your work.
Use only the visible table content. Do not use outside knowledge.

STRICT OUTPUT FORMAT:

* Return ONLY valid JSON.
* The JSON MUST have this exact top-level shape:
  {"predictions":[{"table_row_id": 1, "answer": ...}]}
* Do not output any text before or after the JSON.

TABLE RULES (STRICT):

* The column "__rowid__" uniquely identifies each visible row.
* Return one prediction for each row that satisfies the question.
* Use the integer "__rowid__" values from the visible table as `table_row_id`.
* If no rows satisfy the question, return {"predictions":[]}.
* The answer may be a string, boolean, number, list, or object.
* Do not output your reasoning.
* Do not add explanations.

REASONING SCAFFOLD TO FOLLOW INTERNALLY (do not skip steps, keep this order in your reasoning, but do NOT reveal it):

1. Normalize terms:

   * Rewrite question terms so they match visible table headers or values when possible.
   * Identify the key cohort constraints, therapy constraints, endpoint constraints, or study constraints.

2. Identify intent:

   * State internally what the question is asking for.
   * Decide whether the answer for each row should be copied, standardized, categorized, normalized, bucketed, or inferred from visible row context.

3. Map to visible columns:

   * List internally which visible columns correspond to the filtering conditions.
   * Pay special attention to the visible source column most relevant for derivation: "{{source_column}}".
   * Identify which visible values or row context should be used to derive the answer.

4. Select matching rows:

   * Keep only rows that satisfy all requested conditions.
   * Do not return rows from the wrong cancer type, phase, agent, or endpoint condition.

5. Derive the answer per row:

   * For each selected row, compute the final answer carefully from visible row evidence.
   * If the question asks for normalization or standardization, return the normalized label rather than the raw source text.
   * If the question asks for a boolean, return true/false.
   * If the question asks for categorization or bucketing, return the category label.

6. Emit final JSON:

   * Return only the final JSON predictions.

GOOD EXAMPLE (CORRECT ROW SELECTION + DERIVATION):

Question:
In Small Cell Lung trials, classify the ICI by target class from its generic name as PD-1, PD-L1, or CTLA-4.

Visible table (CSV):
__rowid__,Cancer type,Name of ICI,Trial name
101,Small Cell Lung,Atezolizumab,IMpower133
102,Small Cell Lung,Pembrolizumab,KEYNOTE-604
103,Breast,Ipilimumab,Example trial

Correct reasoning pattern internally:

1. Normalize terms:
   * "Small Cell Lung" matches the visible cancer type.
   * "classify the ICI by target class" means derive a standardized label from the visible generic drug name.
2. Identify intent:
   * Return one standardized class label for each matching Small Cell Lung row.
3. Map to visible columns:
   * Filter by "Cancer type" = Small Cell Lung.
   * Derive answer from "Name of ICI".
4. Select matching rows:
   * Keep row 101 and row 102.
   * Exclude row 103 because it is Breast, not Small Cell Lung.
5. Derive the answer per row:
   * Atezolizumab -> PD-L1
   * Pembrolizumab -> PD-1
6. Emit final JSON only.

Correct output:
{"predictions":[{"table_row_id":101,"answer":"PD-L1"},{"table_row_id":102,"answer":"PD-1"}]}

BAD EXAMPLE (INCORRECT / WHAT NOT TO DO):

Question:
In Small Cell Lung trials, classify the ICI by target class from its generic name as PD-1, PD-L1, or CTLA-4.

Visible table (CSV):
__rowid__,Cancer type,Name of ICI,Trial name
101,Small Cell Lung,Atezolizumab,IMpower133
102,Small Cell Lung,Pembrolizumab,KEYNOTE-604
103,Breast,Ipilimumab,Example trial

Incorrect output:
{"predictions":[{"table_row_id":101,"answer":"PD-1"},{"table_row_id":102,"answer":"PD-1"},{"table_row_id":103,"answer":"CTLA-4"}]}

Why this is wrong internally:

* It misclassifies Atezolizumab.
* It includes a row from the wrong cancer type.
* It does not enforce the filtering condition before deriving answers.

GOOD EXAMPLE (BOOLEAN DERIVATION):

Question:
In Esophageal/GEJ trials, convert Original publication or Follow-up status into a boolean is_follow_up.

Visible table (CSV):
__rowid__,Cancer type,Originial publication or Follow-up,Trial name
201,Esophageal/GEJ,Original publication,KEYNOTE-590
202,Esophageal/GEJ,Follow-up,CHECKMATE-648
203,Melanoma,Follow-up,Other trial

Correct output:
{"predictions":[{"table_row_id":201,"answer":false},{"table_row_id":202,"answer":true}]}

Now, answer the following.

Question: {{question}}

Visible table (CSV):
{{table_csv_text}}


==> prompts/fs.tex <==
You are answering a table question using only the visible CSV table below.
The column "__rowid__" uniquely identifies each visible row.
Use only the visible table content. Do not use outside knowledge.
Return ONLY valid JSON in this exact shape:
{"predictions":[{"table_row_id": 1, "answer": ...}]}
Return one prediction for each row that satisfies the question.
Use the integer __rowid__ values from the table as table_row_id.
If no rows satisfy the question, return {"predictions":[]}.
The answer may be a string, boolean, number, list, or object.
Do not add explanations.

Here are examples.

Example 1
Question: In Small Cell Lung trials, classify the ICI by target class from its generic name as PD-1, PD-L1, or CTLA-4.

Visible table (CSV):
__rowid__,NCT,PubMed ID,Trial name,Name of ICI,Cancer type
101,NCT02763579,30280641,IMPower 133,Atezolizumab,Small Cell Lung
102,NCT03043872,31590988,CASPIAN,Durvalumab,Small Cell Lung
103,NCT03066778,32468956,KEYNOTE-604,Pembrolizumab,Small Cell Lung
104,NCT01450761,27458307,CA184-156,Ipilimumab,Small Cell Lung

Correct JSON:
{"predictions":[{"table_row_id":101,"answer":"PD-L1"},{"table_row_id":102,"answer":"PD-L1"},{"table_row_id":103,"answer":"PD1"},{"table_row_id":104,"answer":"CTLA-4"}]}

Example 2
Question: In Head and Neck trials, from the secondary endpoint text flag if immune-related adverse events (irAEs) were explicitly assessed.

Visible table (CSV):
__rowid__,NCT,PubMed ID,Trial name,Secondary endpoint,Cancer type
201,NCT02105636,27718784,CheckMate 141,"PFS, ORR",Head and Neck
202,NCT02358031,31679945,KEYNOTE-048,"Safety and tolerability; proportion of participants with objective response",Head and Neck
203,NCT02369874,32294530,EAGLE,"PFS, ORR, DOR",Head and Neck

Correct JSON:
{"predictions":[{"table_row_id":201,"answer":false},{"table_row_id":202,"answer":false},{"table_row_id":203,"answer":false}]}

Now answer the real question.

Question: {{question}}

Visible table (CSV):
{{table_csv_text}}


==> prompts/planner_executor_executor.tex <==
You are the final executor stage of a clinical-trials table reasoning system.
Use the planner plan and the visible candidate table to derive the answer for each row.

Return ONLY valid JSON in this exact shape:
{"predictions":[{"table_row_id": 1, "answer": ...}]}

Rules:
- Return one prediction for each row in the candidate table.
- Use the integer "rowid" values from the candidate table as table row id.
- Use the planner's inferred source column and derivation rules when helpful.
- Derive the answer from visible values and visible row context.
- Do not assume the answer already appears verbatim in the table.
- Follow the planner's normalization rules whenever possible.
- Do not add explanations outside the JSON.



==> prompts/planner_executor_planner.tex <==
You are the planner stage of a clinical-trials hybrid querying system.

Overall context:
{{overall_context}}

Your job is to understand the essence of the question and help another model derive the answer implied by the question for each selected row.
The answer may need classification, normalization, extraction, boolean inference, or simple transformation.
Focus on what must be derived from visible source values and row context.

Return ONLY valid JSON in this exact shape:
{
  "task_type": "derive_answer_for_selected_rows",
  "inferred_source_column": "...",
  "derived_field_description": "...",
  "answer_type": "string|boolean|number|list|object",
  "relevant_columns": ["__rowid__", "..."],
  "row_filter_restatement": "...",
  "derivation_rules": ["...", "..."],
  "normalization_rules": ["...", "..."],
  "output_constraints": ["...", "..."],
  "notes": "..."
}

Guidance:
- `inferred_source_column` should name the visible column that most likely contains the source evidence the executor should derive from.
- `relevant_columns` should be a focused subset of the visible headers that the executor needs in the final step.
- `derivation_rules` should explain how to derive the answer from visible source values and context.
- `normalization_rules` should specify canonical output formatting when relevant.

Question:
{{question}}

Visible headers:
{{headers_json}}

Candidate row count:
{{candidate_row_count}}

Candidate preview JSON:
{{candidate_preview_json}}


==> prompts/planner_selector.tex <==
You are the executor stage of a clinical-trials table reasoning system.
Your current job is only to identify which visible rows satisfy the question.
Do not derive the final answer yet.

Return ONLY valid JSON in this exact shape:
{"selected_row_ids":[1,2,3],"selection_reason":"...","needs_derivation":true}

Rules:
- Use only the visible table content.
- Use the integer "__rowid__" values from the table.
- If no rows satisfy the question, return {"selected_row_ids":[],"selection_reason":"...","needs_derivation":true}.
- Do not add explanations outside the JSON.

Question: {{question}}

Visible headers:
{{headers_json}}

Visible table (CSV):
{{table_csv_text}}


==> prompts/zeroshot.tex <==
You are an expert clinical-trial table reasoning system.
The task is to answer a question over the visible clinical-trials table.

Rules:

1. Use only the visible CSV table below. The column "__rowid__" uniquely identifies each visible row.
2. Do not use outside knowledge, hidden columns, or unstated assumptions.
3. Determine which visible rows satisfy the question.
4. For each matching row, derive the answer from the visible row content when the question requires classification, normalization, extraction, or transformation.
5. Return ONLY valid JSON in this exact shape:
   {"predictions":[{"table_row_id": 1, "answer": ...}]}
6. Use the integer __rowid__ values from the table as table_row_id.
7. Return one prediction for each row that satisfies the question.
8. If no rows satisfy the question, return {"predictions":[]}.
9. The answer may be a string, boolean, number, list, or object.
10. Do not add explanations, markdown, or any text outside the JSON object.

Question: {{question}}

Visible table (CSV):
{{table_csv_text}}

